Enhancing Product Safety in E-Commerce with NLP

Ensuring safety of the products offered to the customers is of paramount importance to any e- commerce platform. Despite stringent quality and safety checking of products listed on these platforms, occasionally customers might receive a product that can pose a safety issue arising out of its use. In this paper, we present an innovative mechanism of how a large scale multinational e-commerce platform, Zalando, uses Natural Language Processing techniques to assist timely investigation of the potentially unsafe products mined directly from customer written claims in unstructured plain text. We systematically describe the types of safety issues that concern Zalando customers. We demonstrate how we map this core business problem into a supervised text classification problem with highly imbalanced, noisy, multilingual data in a AI-in-the-loop setup with a focus on Key Performance Indicator (KPI) driven evaluation. Finally, we present detailed ablation studies to show a comprehensive comparison between different classification techniques. We conclude the work with how this NLP model was deployed.

==> acknowledgment.tex <==
\section*{Acknowledgments}
The authors would like to sincerely thank the reviewers for spending their valuable time in 
reviewing and providing constructive comments. We are also grateful to Ralf Herbrich, 
Adrien Renahy, Anthony Brew, Matti Lyra, Svetoslava Ande, and Urs Bergmann for their suggestions, and support
during the work.


==> data_desc.tex <==
\section{Data Description}
\label{section:data_description}
\begin{itemize}
    \item Zalando operates in 18 language markets: German (Germany, Austria, Switzerland), Polish, French (France, Switzerland, Belgium), Dutch (the Netherlands, Belgium), English (UK, Ireland), Italian (Italy, Switzerland), Spanish, Swedish, Danish, Norwegian, Finnish, Czech, Slovak, Estonian, Latvian, Lithuanian, Slovenian and Croatian. 
    \item In each market customers can open a case by submitting a reclamation via reclamation web-form by filling in the order and article details, as well as submitting the free-form text description of reclamation in text field.
    \item The volume of reclamations varies by market, with most almost 80\% of reclamations coming from German, Polish, French and Dutch language markets. 
    \item Reclamations are processed manually by Customer Care agents that forward any reclamation that may refer to a product safety issue to Product Safety specialists who decide if the case needs further inspection. Product Safety specialist 
    \item We use the label provided by Product Safety specialist Therefore our labelled data is both biased and noisy. Biased, since we use only the labels provided by Product Safety specialists which are filtered through Customer Care agents, and that are just a small proportion of the whole volume of reclamations and noisy because it is possible that Customer Care agents miss some genuine product safety cases.
\end{itemize}

\subsection{Text Data}
Here is the description for textual data.


==> discussion.tex <==
\section{Discussion}
\label{section:discussion}
Here is the discussion section.

==> related_work.tex <==
\section{Related Work}
\label{section:related}
%There are multiple (rather overlapping) lines of works that are relevant 
%to our work \textit{i.e.,} text classification in general, transfer 
%learning, and meta-learning in NLP.

% \noindent{\textbf{Text classification.}} Text classification began with knowledge-driven, rule-based systems, 
% followed by approaches that rely on bag-of-words representations and feature engineering \cite{baker1998distributional,scott1998text,rogati2002high}
% to data-driven, distributed word representations (word embeddings) learned in self- or unsupervised manner as integral part of deep neural networks \cite{pennington2014glove,mikolov2013distributed,Peters:2018}. 
% These representations have been widely adopted for various text classification tasks 
% with different neural architectures \cite{kim2014convolutional,rocktaschel2015,liu2016}.
% Transformer-based models, that take advantage of self- and cross-attention mechanisms have recently shown 
% significant improvement over other architectures across wide range of NLP tasks, 
% including text classification\footnote{All the top teams in \url{gluebenchmark.com/leaderboard} 
% use transformer-based models at the time of writing.} \cite{vaswani2017attention,devlin2019bert,yang2019xlnet}.

\noindent{\textbf{Transfer learning.}} Transferring knowledge from one learned task to another relies on 
exploiting similarities across tasks \textit{e.g,} for question answering, sentiment analysis, and passage re-ranking among others
\cite{min2017question,severyn2015unitn,howard2018universal,nogueira2019passage,dai2019deeper}. Here the focus 
%of transfer learning in NLP 
is mainly on transferring knowledge from self- or unsupervised tasks (language modelling) that can exploit large corpora 
to supervised tasks (like text classification) for which limited labelled data exists. In this work, we are 
interested in transferring knowledge from one supervised task to another, with varying amount of semantic task 
similarity and data distribution similarity. In that respect, a unified text-to-text transformer model 
\cite{raffel2019exploring} which tackles all NLP problems (\textit{e.g.} translation, classification, 
regression) as sequence-to-sequence problems is the most related to our work. We can cast the text classification 
in that context as prediction of one token with two possible values (0 and 1).

\noindent{\textbf{Zero/few shot learning.}} The problem of \textit{zero shot}, and 
\textit{few shot} learning has lately been proposed in the context of NLP \cite{han2018fewrel,geng2019induction}
using meta-learning. Model agnostic meta-learning (MAML) has been explored to tackle tasks 
with disjoint label spaces \cite{bansal2019learning}. However, these models are not capable of making
zero shot predictions. To the best of our knowledge, the only viable zero shot abilities in NLP has 
been shown in the literature by using pre-trained GPT-2 model \cite{puri2019zero}. 
Similar to this work, it utilizes descriptors of the task at hand in natural language, 
but there it is formulated as question answering problem, rather than as classification problem as we do.
%it is done in this work.

% Decomposition of multi-class classification into multiple binary classification  
% was studied in early machine learning literature. It involves training 
% either \textit{e.g.,} $M$ separate classifiers in One-versus-All (OVA), 
% \textit{or} $\frac{M(M-1)}{2}$ classifiers in All-versus-All (AVA) 
% setting \cite{aly2005survey,allwein2000reducing}. These works motivated towards 
% implementing multi-class classifiers with early robust binary classifiers such as SVM 
% \cite{cortes1995support}. In contrast, we define a function approximation 
% method to unify many classification problems and yields a \textit{single} 
% model to perform predictions after due training.
